Pushing Rendering Boundaries: Hard Gaussian Splatting

3D Gaussian Splatting (3DGS) has demonstrated impressive Novel View Synthesis (NVS) results in a real-time rendering manner. During training, it relies heavily on the average magnitude of view-space positional gradients to grow Gaussians to reduce rendering loss. However, this average operation smooths the positional gradients from different viewpoints and rendering errors from different pixels, hindering the growth and optimization of many defective Gaussians. This leads to strong spurious artifacts in some areas. To address this problem, we propose Hard Gaussian Splatting, dubbed HGS, which considers multi-view significant positional gradients and rendering errors to grow hard Gaussians that fill the gaps of classical Gaussian Splatting on 3D scenes, thus achieving superior NVS results. In detail, we present positional gradient driven HGS, which leverages multi-view significant positional gradients to uncover hard Gaussians. Moreover, we propose rendering error guided HGS, which identifies noticeable pixel rendering errors and potentially over-large Gaussians to jointly mine hard Gaussians. By growing and optimizing these hard Gaussians, our method helps to resolve blurring and needle-like artifacts. Experiments on various datasets demonstrate that our method achieves state-of-the-art rendering quality while maintaining real-time efficiency.

==> tab/mip360_db.tex <==

\begin{tabular}{l|ccc|ccc}
\toprule
Dataset & \multicolumn{3}{c|}{Mip-NeRF360} & \multicolumn{3}{c}{Deep Blending} \\
Method$\,|\,$Metric & PSNR \(\uparrow\) & SSIM \(\uparrow\) & LPIPS \(\downarrow\) & PSNR \(\uparrow\) & SSIM \(\uparrow\) & LPIPS \(\downarrow\) \\
\midrule
Plenoxels~\cite{fridovich2022plenoxels} & 23.08 & 0.626 & 0.463 & 23.06 & 0.795 & 0.510 \\ 
INPG~\cite{muller2022instant} & 25.59 & 0.699 & 0.331 & 23.62 & 0.797 & 0.423 \\
Mip-NeRF360~\cite{barron2022mip} & 27.69 & 0.792 & 0.237 & 29.40 & 0.901 & 0.245 \\
3DGS~\cite{kerbl20233d} & 27.71 & 0.825 & 0.202 & 29.46 & 0.899 & 0.247 \\
Mip-Splatting~\cite{yu2024mip} \\
mini-Splatting~\cite{fang2024mini} & 27.51 & 0.831 & 0.176 & 29.88 & 0.906 & 0.211 \\
Scaffold-GS~\cite{lu2024scaffold} & 27.98 & 0.825 & 0.208 & 30.23 & 0.907 & 0.245 \\
Pixel-GS~\cite{zhang2024pixel} & 27.88 & 0.834 & 0.176 & 28.88 & 0.892 & 0.251 \\
\midrule
\textbf{MH-GS (Ours)} & 28.15 & 0.830 & 0.176 & 30.35 & 0.908 & 0.230 \\
\bottomrule
\end{tabular}
